Bayesian Imaging With Data-Driven Priors Encoded by Neural Networks: Theory, Methods, and Algorithms

This paper proposes a new methodology for performing Bayesian inference in imaging inverse problems where the prior knowledge is available in the form of training data. Following the manifold hypothesis and adopting a generative modelling approach, we construct a data-driven prior that is supported on a sub-manifold of the ambient space, which we can learn from the training data by using a variational autoencoder or a generative adversarial network. We establish the existence and well-posedness of the associated posterior distribution and posterior moments under easily verifiable conditions, providing a rigorous underpinning for Bayesian estimators and uncertainty quantification analyses. Bayesian computation is performed by using a parallel tempered version of the preconditioned Crank-Nicolson algorithm on the manifold, which is shown to be ergodic and robust to the non-convex nature of these data-driven models. In addition to point estimators and uncertainty quantification analyses, we derive a model misspecification test to automatically detect situations where the data-driven prior is unreliable, and explain how to identify the dimension of the latent space directly from the training data. The proposed approach is illustrated with a range of experiments with the MNIST dataset, where it outperforms alternative image reconstruction approaches from the state of the art. A model accuracy analysis suggests that the Bayesian probabilities reported by the data-driven models are also remarkably accurate under a frequentist definition of probability.

==> ex_shared.tex <==

\usepackage{epstopdf}
\usepackage{algorithmic}
\usepackage{graphicx,epstopdf} %
\usepackage[symbol*]{footmisc}

\ifpdf
   \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
   \DeclareGraphicsExtensions{.eps}
\fi

\newcommand{\creflastconjunction}{, and~}

\newsiamremark{remark}{Remark}
\newsiamremark{hypothesis}{Hypothesis}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{claim}{Claim}



\headers{Bayesian imaging with data-driven priors}{M. Holden, M. Pereyra, K. Zygalakis}
\title{Bayesian imaging with data-driven priors encoded by neural networks: theory, methods, and algorithms~\thanks{Submitted to the editors DATE.
\funding{MH was supported by The Maxwell Institute Graduate School in Analysis and its Applications, a Centre for Doctoral Training funded by the UK Engineering and Physical Sciences Research Council (grant EP/L016508/01), the Scottish Funding Council, Heriot-Watt University and the University of Edinburgh.  MP was supported by UKRI EPSRC (EP/T007346/1). KCZ was supported by a Leverhulme Research Fellowship. Computer experiments for this work ran on a Titan Xp GPU donated by NVIDIA.}}}


\footnotetext[1]{School of Mathematical and Computer Sciences, 
Heriot-Watt University, Edinburgh, Scotland}
\footnotetext[2]{School of Mathematics, University of Edinburgh, 
Edinburgh, Scotland}
\footnotetext[3]{Maxwell Institute for Mathematical Sciences, Bayes 
Centre, 47 Potterrow, Edinburgh, Scotland}



\author{Matthew Holden\footnotemark[1]\ \footnotemark[2]\ \footnotemark[3]
\and Marcelo Pereyra\footnotemark[1]\ \footnotemark[3]
\and Konstantinos C. Zygalakis\footnotemark[2]\ \footnotemark[3]}


\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}


\makeatletter
\newcommand*{\addFileDependency}[1]{%
  \typeout{(#1)}%
  \@addtofilelist{#1}%
  \IfFileExists{#1}{}{\typeout{No file #1.}}%
}
\makeatother

\newcommand*{\myexternaldocument}[1]{%
    \externaldocument{#1}%
    \addFileDependency{#1.tex}%
    \addFileDependency{#1.aux}%
}

